Temperature inhomogeneities in Mrk71 can not be discarded

In a very recent work, [1] claim that the scenario of temperature inhomogeneities proposed by [2] ($t2$ > 0) is not able to explain the O$^{2+}$/H$^{+}$ abundance discrepancy observed between the calculations based on the optical [OIII] collisional excited lines (CELs) and the OII recombination lines (RLs) in the star forming galaxy Mrk71. In this work, we show that conclusions of [1] depend on several assumptions on the absolute flux calibration, reddening correction and the adopted electron density. In fact, using the data of [1] in a different way and even considering their 1{\sigma} uncertainties, it is possible to reach the opposite conclusion, consistent with $t2$ = $0.097 ^{+0.008}_{-0.009}$. Therefore, the existence of temperature inhomogeneities causing the O$^{2+}$/H$^{+}$ abundance discrepancy in Mrk71 can not be ruled out.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


